Interpolation-Based GR(1) Assumptions Refinement

This paper considers the problem of assumptions refinement in the context of unrealizable specifications for reactive systems. We propose a new counterstrategy-guided synthesis approach for GR(1) specifications based on Craig's interpolants. Our interpolation-based method identifies causes for unrealizability and computes assumptions that directly target unrealizable cores, without the need for user input. Thereby, we discuss how this property reduces the maximum number of steps needed to converge to realizability compared with other techniques. We describe properties of interpolants that yield helpful GR(1) assumptions and prove the soundness of the results. Finally, we demonstrate that our approach yields weaker assumptions than baseline techniques, and finds solutions in case studies that are unsolvable via existing techniques.

==> sections/discussion.tex <==
\section{Discussion}
\label{sec:Discussion}
\subsection{Targeting unrealizable cores}
The evaluation shows that our approach automatically selects variables that need to be constrained in order to reach realizability. In particular, all the intermediate refinements eliminate precisely a cause of unrealizability, consisting of the set of minimally unfulfillable guarantees from which a counterstrategy has been computed. We note that the returned variables in the AMBA02 example ($\hready$ and $\hbusreqone$) are a subset of the variables that the authors in \cite{Alur2013} suggest to use in order to instantiate the refinement templates. 
%The additional test conducted on AMBA02 shows that variable selection is critical in the refinement problem: in fact, not all template instantiations remove the cause of unrealizability from a minimally unfulfillable set of guarantees; removing this is a necessary condition for achieving realizability \cite{Cimatti2008a}.

Helpfulness of intermediate refinements is a desirable condition for reducing the convergence rate of the algorithm. When this holds, then the expected tree depth $d$ (see Sect.~\ref{sec:Convergence}) is reduced to $O(n_g)$, where $n_g$ is the number of minimally unfulfillable subsets of guarantees. In the Lift controller and AMBA-AHB case studies such condition is met consistently. In ColorSort only 49\% of the nodes fulfill this property.
\textbf{TODO: Check whether this percentage is consistently higher than that of Alur's}

%\subsection{Number of unrollings}
%We further define an upper bound to the number of unrollings needed to reach the termination condition as of Sect.~\ref{subsec:Unrolling}. Every unrolling iteration produces an interpolant which is either the same as the previous iteration, or contains the description of one more state in the counterplay. In the worst case, without unrolling the interpolant describes just the initial state; after the first unrolling it contains a state component for the first transient state $s^{trans}_1$; it is iteratively strengthened by one more state component until it describes all the transient states and the first replica of the unrolled states $s^{unr}_{j,1}$ for each $j$. In the following unrolling step, the interpolant  contains the component of $s^{unr}_{1,2}$, which is such that $\lambda'(\unrolledstate{1}{2})=\lambda'(\unrolledstate{1}{1})$: interpolation produces an equivalent refinement to the previous step, and therefore the procedure terminates.
%%Figure~\ref{fig:UnrollingBound} pictures this situation.
%%\begin{figure}
%%\centering
%%\includegraphics[width=0.7\linewidth]{figs/UnrollingBound}
%%\caption{Bound for the unrolling loop. $I_3$ does not produce further refinements since it includes the description of a state which is a replica of $I_2$}
%%\label{fig:unrollingbound}
%%\end{figure}
%%
%The maximum number of unrollings  before reaching the termination condition  is:
%%\begin{equation}
%$u_{C,MAX} = |S|$
%%\end{equation}
%where $|S|$ is the number of states in $\pi_C$.

\subsection{Comparison with existing approaches}
Our approach extracts weaker refinements that those of  \cite{Alur2013}. The reason is that \cite{Alur2013} uses templates that are true over all paths of a counterstrategy, while our approach  requires them to be true in a single counterplay. More specifically, an invariant template used in \cite{Alur2013} has the form $\always \lnot q \lor \next \left(\bigwedge_{q' \in \textit{Next}(q)} \lnot q'\right)$, where $q$ and $q'$ indicate states in a counterstrategy and $Next(q)$ is the set of successor states of $q$; our approach extracts invariants of the form $\always \lnot q \lor \lnot q'$ for a $q' \in Next(q)$, which is implied by the former one, provided that they use the same  variables set for $q$ and $q'$.

We notice that in principle our approach may generate assumptions containing only output variables. This happens if some state component in the interpolant contains only output variables. Those are valid GR(1) formulae according to the definition, although hardly interpretable as constraints on the environment. Existing approaches circumvent the problem by allowing only input variables in their refinements \cite{Alur2013,Alur2015}: however, in this way valid assumptions are also excluded. In our AMBA04 case study, one of the computed assumptions was $\always ((\lnot hmaster0 \land hbusreq1) \rightarrow \next (\lnot hbusreq1))$, where $hmaster0 \in \outy$ and $hbusreq1 \in \inx$. This assumption would not have been computed with that restriction.
